Action Anticipation for Collaborative Environments: The Impact of Contextual Information and Uncertainty-Based Prediction

To interact with humans in collaborative environments, machines need to be able to predict (i.e., anticipate) future events, and execute actions in a timely manner. However, the observation of the human limb movements may not be sufficient to anticipate their actions unambiguously. In this work, we consider two additional sources of information (i.e., context) over time, gaze, movement and object information, and study how these additional contextual cues improve the action anticipation performance. We address action anticipation as a classification task, where the model takes the available information as the input and predicts the most likely action. We propose to use the uncertainty about each prediction as an online decision-making criterion for action anticipation. Uncertainty is modeled as a stochastic process applied to a time-based neural network architecture, which improves the conventional class-likelihood (i.e., deterministic) criterion. The main contributions of this paper are four-fold: (i) We propose a novel and effective decision-making criterion that can be used to anticipate actions even in situations of high ambiguity; (ii) we propose a deep architecture that outperforms previous results in the action anticipation task when using the Acticipate collaborative dataset; (iii) we show that contextual information is important to disambiguate the interpretation of similar actions; and (iv) we also provide a formal description of three existing performance metrics that can be easily used to evaluate action anticipation models.Our results on the Acticipate dataset showed the importance of contextual information and the uncertainty criterion for action anticipation. We achieve an average accuracy of 98.75% in the anticipation task using only an average of 25% of observations.

==> vitae.tex <==


\vspace{2cm}
\par\noindent 
\parbox[t]{\linewidth}{
\noindent\parpic{\includegraphics[height=1.5in,width=1in,clip,keepaspectratio]{images/clebeson_canuto.jpeg}}
\noindent 
\textbf{Clebeson Canuto} is a Ph.D. student in Electrical Engineering at Federal University of Esp\'irito Santo, Brazil, advised by Dr. Raquel Vassallo. He received his M.S. in Computer Science in 2016 from Federal University of Sergipe, Brazil, advised by Dr. Eduardo Freire. He earned his B.S. in Information System in 2013 from University Tiradentes, Brazil. He is currently a visiting student at Computer and Robot Vision Laboratory (Lisbon, Portugal), under the supervision of Dr. Jos\'e Santos-Victor. His research interests are mainly in computer vision, deep learning and human-robot interaction.
}


\par\noindent 
\parbox[t]{\linewidth}{
\noindent\parpic{\includegraphics[height=1.5in,width=1in,clip,keepaspectratio]{images/plinio_moreno.jpeg}}
\noindent 
\textbf{Plinio Moreno} is a Research Scientist at Insitute for Systems and Robotics (Lisbon, Portugal). He obtained the M.Sc. in Computer Science by the Universidad de los Andes (Bogot\'a, Colombia) in 2002 and completed the PhD in Electrical and Computers Engineering by the Instituto Superior T\'ecnico (Lisbon, Portugal) in 2008. He has more than 40 published papers in the areas of computer vision, pattern recognition and robotics, with 711 citations and h-index 11. He has been involved in three Framework Programme (FP) European research projects: Context Aware Vision using Image-based Active Recognition (CAVIAR-FP6), Ubiquitous Networking Robotics in Urban Settings (URUS-FP6) and Flexible Skill Acquisition and Intuitive Robot Tasking for Mobile Manipulation in the Real World (First-MM-FP7).
}


\par\noindent 
\parbox[t]{\linewidth}{
\noindent\parpic{\includegraphics[height=1.5in,width=1in,clip,keepaspectratio]{images/jorge-aching.jpeg}}
\noindent 
\textbf{Jorge Samatelo} has a degree in Electronic Engineering from the National University of San Marcos (2001), Peru,a M.S. in Electrical Engineering from Federal University of Esp\'{i}rito Santo (2007), Brazil, and a Ph.D. in Electrical Engineering from Federal University of Esp\'{i}rito Santo (2012), Brazil. He is currently Associate Professor at the Federal University of Esp\'{i}rito Santo. His areas of expertise are image processing, computer vision, and deep learning.
}


\par\noindent 
\parbox[t]{\linewidth}{
\noindent\parpic{\includegraphics[height=1.5in,width=1in,clip,keepaspectratio]{images/raquel_vassallo.jpg}}
\noindent 
\textbf{Raquel Vassallo} received the M.Sc. degree in automation and the Ph.D. degree in electrical engineering from the Federal University of Espirito Santo (UFES), Brazil, in 1998 and 2004, respectively. Her Ph.D. dissertation was on computer vision applied to mobile robotics in cooperation with the Instituto Superior T\'ecnico, Lisbon, Portugal. She is currently an Associate Professor with the Electrical Engineering Department, UFES. Her research is mainly focused on computer vision for mapping, robot navigation, intelligent spaces, and mobile robotics.
} 


\par\noindent 
\parbox[t]{\linewidth}{
\noindent\parpic{\includegraphics[height=1.5in,width=1in,clip,keepaspectratio]{images/jose_santos_victor.jpg}}
\noindent 
\textbf{Jos\'e Santos-Victor} received the Ph.D. in Electrical and Computer Engineering from Instituto Superior T\'ecnico (IST), Lisbon, Portugal, in 1995. He is currently Full Professor at IST, Director of the Institute for Systems and Robotics (ISR-Lisboa) and head of the Computer and Robot Vision Laboratory (VisLab). He is the scientific responsible for IST in many European and national research projects in cognitive and bio-inspired computer vision and robotics. He published more than 300 articles in international journals and conferences (h-index 37).
}



